Machine Learning-enhanced Efficient Spectroscopic Ellipsometry Modeling

Over the recent years, there has been an extensive adoption of Machine Learning (ML) in a plethora of real-world applications, ranging from computer vision to data mining and drug discovery. In this paper, we utilize ML to facilitate efficient film fabrication, specifically Atomic Layer Deposition (ALD). In order to make advances in ALD process development, which is utilized to generate thin films, and its subsequent accelerated adoption in industry, it is imperative to understand the underlying atomistic processes. Towards this end, in situ techniques for monitoring film growth, such as Spectroscopic Ellipsometry (SE), have been proposed. However, in situ SE is associated with complex hardware and, hence, is resource intensive. To address these challenges, we propose an ML-based approach to expedite film thickness estimation. The proposed approach has tremendous implications of faster data acquisition, reduced hardware complexity and easier integration of spectroscopic ellipsometry for in situ monitoring of film thickness deposition. Our experimental results involving SE of TiO2 demonstrate that the proposed ML-based approach furnishes promising thickness prediction accuracy results of 88.76% within +/-1.5 nm and 85.14% within +/-0.5 nm intervals. Furthermore, we furnish accuracy results up to 98% at lower thicknesses, which is a significant improvement over existing SE-based analysis, thereby making our solution a viable option for thickness estimation of ultrathin films.

==> Sections/relatedWork.tex <==
\section{Related Work}
\label{sec:relatedwork}

==> Sections/results_OG.tex <==
\section{Experiments}
\label{sec:results}

\subsection{Experimental Setup}
\label{sec:setup}

The substrates used for deposition were silicon with native oxide. They were ultrasonically cleaned in a mixture of isopropyl alcohol (IPA) and deionized H2O and dried with compressed air. The films were deposited using a Fiji Gen2 ALD System from Veeco®. The films grown were ZnO, Al\textsubscript{2}O\textsubscript{3}, and TiO\textsubscript{2}. The processes consisted of alternate pulses of each film’s precursor, diethyl zinc (DEZ, Sigma Aldrich, CAS:557-20-0 ≥ 52 wt. \% in hexane), trimethyl aluminum (TMA 97\%, Sigma Aldrich), and titanium tetraisopropoxide (TTIP 97\%, Sigma Aldrich), respectively followed by deionized water.

The film thicknesses were tracked using an M-2000 spectroscopic ellipsometer (SE) from J. A. Woollam®. The light source and detector mount to the Fiji ALD system with 2.75” conflat flanges and quartz windows. The windows are purged, protecting them from deposition, with 50 sscm of gaseous argon. The angle of incidence of the light on the sample was 69.5°. The wavelengths used for data acquisition ranged from 271 nm – 1688 nm, for a total of 661 different wavelengths per scan. The change in polarization from incident light to the reflected light was measured for each film. The quantities $\Psi$ and $\Delta$ are the raw data obtained from the SE, and they are representative of the change in polarization. Models were then used to fit the $\Psi$ and $\Delta$ as functions of wavelength to obtain film thickness.

Optical models for each film were created using the CompleteEase software from J.A. Woollam®. The model for the ZnO film was a general oscillator model with a combination of a UV pole ($\varepsilon$1) and a single gaussian peak ($\varepsilon$2) to make the complex dielectric function ($\varepsilon$1 + i $\varepsilon$2) (ref). The model for the Al\textsubscript{2}O\textsubscript{3} is given by a Cauchy-based model (ref). The model for TiO\textsubscript{2} was a Cauchy-based model (ref) as well. These models are part of a physics-based approach to estimate film thickness using SE data. To estimate film thickness via machine learning, the large amount of data generated by \textit{in situ} SE must be used to train an algorithm. The details of this process are given below.


\subsection{Results}
\label{subsec:results}

\subsubsection{ZnO Ellipsometry}
\label{subsubsec:znoresults}

The first case study compares the performance of the various ML algorithms, as demonstrated in Figure\ref{fig:znoallclassifiers}. The percent accuracy (Y-axis) illustrates the probability of each model to classify a datapoint into one of the fifteen classes of the curated dataset to within ± 1.5 nm accuracy, i.e., level-1 classification. kNN furnishes the best accuracy score, where each datapoint is classified with a confidence of 87.54\% using five neighbors~\textcolor{orange}{cite here}. SVM, DT, and RF report acceptable results, comparable to kNN, of 83.77\%, 84.54\%, and 86.79\%, respectively. SVM uses a radial basis function of degree three as its kernel, along with a regularization coefficient of value 1. RF is an ensemble of decision trees, and like DT, requires a minimum of two samples to split an internal node. The maximum depth of the tree is not specified in either algorithm, implying that the tree can expand until all datapoints are accounted for. In this experiment, we consider 40 trees in RF. LR, on the other hand, uses a regularization coefficient of value 1 and Limited-memory Broyden–Fletcher–Goldfarb–Shanno (lbfgs) optimization technique36 to calculate the parameter weights that minimize the cost function.

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{Figures/ZnO/1_ZnO_AllClassifiers.png}
\caption{Accuracy results of various Machine Learning classifiers for ZnO spectroscopic ellipsometry data.}
 \label{fig:znoallclassifiers}
\vspace{-0.1in}
\end{figure}

LR performs the worst among all the models, producing a score of 40.74\%. This can be attributed to LR being inept at solving non-linear problems owing to its linear decision surface, the requirement of having an exhaustive dataset, and its sensitivity of outliers in the dataset. Owing to its low accuracy score, LR is not considered for future experiments. Additionally, SVM too is excluded from subsequent case studies for two reasons, the first being its high training time and the second its sub-par classification performance.

The second case study evaluates the performances of the three best algorithms, DT, RF and kNN, with increasing granularity in the prediction of film thickness. These results assume importance from a process perspective since it is important to understand the uncertainty in accuracy (i.e., delta thickness) that is inherently present in a ML algorithm and the uncertainty that is propagated as a function of the true physical thickness of the film.

Accordingly, accuracy scores of each model are as illustrated in Figure~\ref{fig:znoimproved} at both level-1 and level-2. We have updated the hyperparameters of the models to bolster classification performance of each model. Increasing the number of neighbors from 5 to 21 improves the performance of kNN from 87.54\% (as shown in Figure~\ref{fig:znoallclassifiers}) to 88.65\% resulting in an enhancement of 1.11\%. The number of trees in RF is increased from 40 to 100, which furnishes an accuracy of 87.25\% vs. 86.79\%. DT retains the same set of hyperparameters as before, which were optimized to produce best performance, and thus produces the same accuracy score of 84.54\%.  

\begin{figure}[t!]
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/2_ZnO_ImprovedModels.png}
    \caption{}
    \label{fig:znoimproved}
\end{subfigure}

\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/3_ZnO_kNN_Level1.png}
    \caption{}
    \label{fig:znoimprovedlevel1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/4_ZnO_kNN_Level2.png}
    \caption{}
    \label{fig:znoimprovedlevel2}
\end{subfigure}
\caption{(a) Accuracy results of the improved Machine Learning classifiers for ZnO spectroscopic ellipsometry data. (b) Variation of accuracy of kNN classifier with classes for ZnO spectroscopic ellipsometry data. (c) Variation of accuracy of kNN model with thickness for ZnO spectroscopic ellipsometry data.}
\label{fig:znoimprovedmodels_three}
\end{figure}

Apart from refining the models, we also analyze their level-2 accuracy scores. It is intuitive to understand how level-1 classification (wider, 3 nm range) may result in higher accuracy compared to level-2 classification (narrower, 1 nm range). As depicted in Figure~\ref{fig:znoimproved}, kNN again furnishes the best results of 73.83\%, while RF and DT produce scores of 71.56\% and 67.45\%, respectively.  

Since these results reflect the overall classification performance, averaged over all classes and subclasses, there is no information regarding the accuracy scores at specific classes or thicknesses. Hence, we next examine level-1 accuracy and level-2 accuracy by analyzing model performance at each class and thickness, respectively.  

Figure~\ref{fig:znoimprovedlevel1} illustrates the accuracy of kNN at all classes, and as evident from it, we generally witness reduced accuracy scores at classes comprising higher thicknesses. While class 0 ([1-3] nm) has the maximum accuracy of 98.58\%, class 14 ([43,44] nm) is associated with the minimum accuracy of 53.36\%. There is a considerable reduction in accuracy of around 30\%, which can mainly be attributed to the fact that class 14 encompasses only two subclasses ([43-44] nm), unlike the other classes, which consist of three subclasses. Moreover, since the ALD process is terminated at 51.17 min, as soon as a film of 44 nm thickness is obtained, we have access to limited datapoints for this thickness. Next, we increase the granularity and examine kNN classification performance at each thickness, as depicted in Figure~\ref{fig:znoimprovedlevel2}. The accuracy values of the model range between 97.78\% for 1 nm and 3.85\% for 44 nm. Although the general trend is negative, there are a few outliers (such as 39 nm and 42 nm) that produce high accuracy scores. The performance degradation at higher thicknesses may be attributed to the amplification of spectral features in $\Psi$ and $\Delta$, (i.e., peaks and valleys in \textcolor{orange}{Figure 3A, B)} which hinder the learning stage of the models and degrade their classification performance.

% \begin{figure}[t!]
% \centering
%%\subfloat[]{\label{main:c}\includegraphics[scale=.5]{Figures/2_ZnO_ImprovedModels.png}}
% \subfloat[]{\label{main:c}\includegraphics[width=\linewidth]{Figures/2_ZnO_ImprovedModels.png}}
% \begin{minipage}{.5\linewidth}
% \centering
% \subfloat[]{\label{main:a}\includegraphics[width=0.5\linewidth]{Figures/3_ZnO_kNN_Level1.png}}
% \end{minipage}%
% \begin{minipage}{.5\linewidth}
% \centering
% \subfloat[]{\label{main:b}\includegraphics[width=0.5\linewidth]{Figures/4_ZnO_kNN_Level2.png}}
% \end{minipage}\par\medskip
% \caption{my fig}
% \label{fig:main}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/2_ZnO_ImprovedModels.png}
% \caption{Accuracy results of the improved Machine Learning classifiers for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoimprovedmodels}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/3_ZnO_kNN_Level1.png}
% \caption{Variation of accuracy of kNN classifier with classes for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znolevel1}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/4_ZnO_kNN_Level2.png}
% \caption{Variation of accuracy of kNN model with thickness for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znolevel2}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/5_ZnO_Downsampling_Acc.png}
    \caption{}
    \label{fig:znodowsampling_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/6_ZnO_Downsampling_AccDrop.png}
    \caption{}
    \label{fig:znodowsampling_accdrop}
\end{subfigure}
\caption{(a) Random downsampling results of kNN classifier for ZnO spectroscopic ellipsometry data. (b) Accuracy drop results of the kNN classifier for random downsampling of ZnO spectroscopic ellipsometry data.}
\label{fig:downsamplingresults}
\end{figure}

The third case study describes the results of downsampling data, i.e., random $\Psi$ and $\Delta$ values are removed from the curated dataset. Here, we seek to understand how limited spectroscopic data might impact ML prediction accuracy. In the ultimate limit, where only one wavelength (as is the case for single wavelength ellipsometry) is present, might ML accurately predict film thickness? The results assume importance because limited data might indicate avenues for faster data acquisition, reduced hardware complexity (i.e., costs) and therefore, easier integration of SE for \textit{in situ} monitoring of thin film deposition processes, in general. 

The downsampling rate is varied between 0 and 90\% and the performance of the best performing algorithm – the kNN algorithm, is evaluated on the downsampled dataset. Figure~\ref{fig:znodowsampling_acc} depicts the variation of level-1 and level-2 accuracy at different downsampling rates. The level-1 accuracy is generally resilient to donwnsampling, varying between 88.65\% at 0\% and 85.67\% at 85\%, witnessing a maximum accuracy drop of 2.98\%. The level-2 accuracy varies from 73.83\% at 0\% downsampling to 65.46\% at 90\% downsampling. This is an important result as it indicates that thickness prediction via ML can be effectively accurate to within ± 1.5 nm uncertainty (i.e., level-1) of a ZnO film $\leq44 nm$, even if 90\% of the spectral data is eliminated.  

On the other hand, Figure~\ref{fig:znodowsampling_accdrop} shows that downsampling induces a larger degradation in level-2 accuracy. This is equivalent to 8.37\% drop in classification accuracy of the kNN model. However, the accuracy drops are relatively low at both levels until 50\% downsampling. The performance degradation at level-1 and level-2 for 50\% downsampling rate is 0.54\% and 2\%, respectively. These results are indicative of possible redundancy in the dataset with regards to $\Psi$ and $\Delta$ samples. 

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/5_ZnO_Downsampling_Acc.png}
% \caption{Random downsampling results of kNN classifier for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znodownsampling}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/6_ZnO_Downsampling_AccDrop.png}
% \caption{Accuracy drop results of the kNN classifier for random downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znodownsamplingdrop}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/7_ZnO_Downsampling_Acc_Level1.png}
    \caption{}
    \label{fig:znodownsamling_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/8_ZnO_Downsampling_Acc_Level2.png}
    \caption{}
    \label{fig:znodownsamling_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for random downsampling of ZnO spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for random downsampling of ZnO spectroscopic ellipsometry data.}
\label{fig:randomdownsamplingresults}
\end{figure}

We further study the variation of level-1 accuracy and level-2 accuracy with thickness at select downsampling rates of 10\%, 30\%, 50\%, 70\%, and 90\%. Figure~\ref{fig:znodownsamling_level1} shows the level-1 accuracy at different classes (each bin with 3 nm thickness) and Figure~\ref{fig:znodownsamling_level2} the level-2 accuracy at different thickness values. From these graphs, it is evident that the classification performance of kNN degrades at higher thicknesses, irrespective of the random downsampling rate. For example, with 90\% downsampling of SE data, level-1 prediction accuracy drops from 97.01\% for a thickness in bin [4 nm - 6 nm] to 77.55\% for a thickness in bin [40 nm - 42 nm]. Thus, it is the actual physical thickness of the film predicted using ML that can make a difference to the predictive accuracy. This result bodes well for ML algorithms to predict thickness of ultrathin films ($\leq10 nm$) which is always a challenge for SE data analysis. Finally, it can be inferred that the dataset has redundancy that can be eliminated without inducing significant performance degradation. Hence, this motivates us to pursue selective downsampling and explore the connection, if any, between specific $\Psi$ and $\Delta$ samples and classification accuracy.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/7_ZnO_Downsampling_Acc_Level1.png}
% \caption{Variation of accuracy of kNN classifier with classes for random downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znodownsamplinglevel1}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/8_ZnO_Downsampling_Acc_Level2.png}
% \caption{Variation of accuracy of kNN model with thickness for random downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znodownsamplinglevel2}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/9_ZnO_SelectiveDownsampling_Acc.png}
    \caption{}
    \label{fig:selectiveds_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/11_ZnO_CompressionSavings.png}
    \caption{}
    \label{fig:selectiveds_compression}
\end{subfigure}
\caption{(a) Selective downsampling results of kNN classifier for ZnO spectroscopic ellipsometry data. (b) Variation of compression with number of samples for ZnO spectroscopic ellipsometry data.}
\label{fig:selectivedsresults}
\end{figure}

The ultimate objective of an ML algorithm would be to determine thickness from minimal, perhaps few and discrete, wavelength based ellipsometry data. Therefore, the fourth case study involves selective (i.e., non-random) downsampling of $\Psi$ and $\Delta$ values in the curated dataset. We select the first ‘N’ samples from each class and subclass, starting from 271 nm and up, while eliminating the rest. This is shown in Figure~\textcolor{orange}{include figure} which serves to remind the reader of the $\Psi$ and $\Delta$ values of a single spectrum (i.e., related to a fixed thickness). Features such as peaks and valleys appear in the spectra for wavelengths $\leq500 nm$. It is important to note that the $\Psi$ and $\Delta$ are experimentally measured raw data and no modeling effort has been expended to modify the data.  

In this analysis, we consider N ranging from 100 to 300, in step sizes of 50. This corresponds to a spectral window from 271 nm to 427 nm for the first 100, and from 271 nm to 743 nm for first 300, in step sizes of 76 nm. From Figure~\ref{fig:znoselectivedscompression}, an estimate can be made that the first – 300 data points still constitutes a fraction (45.39\%) of the total data collected. 

This downsampled dataset is utilized to train and evaluate kNN, which, in the previous three case studies, has furnished the best results. Figure~\ref{fig:selectiveds_acc} shows the variation of level-1 and level-2 classification accuracy scores. While we obtain the lowest scores of 78.25\% at level-1 and 67.13\% at level-2 for the first 100 samples, improved classification performance is produced at higher values of N. The best level-1 accuracy and level-2 accuracy are 88.63\% and 80.04\%, which are furnished when the first 250 and 300 samples, respectively, constitute the dataset (opposed to 88.65\% level-1 and 73.87\% level-2 accuracies when no downsampling is performed, as shown in Figure~\ref{fig:znoimprovedmodels_three}). This approach of selective downsampling provides results that exceed the baseline accuracy scores of the kNN model, by 6.21\% at level-2.

Another benefit of selective downsampling is illustrated in Figure~\ref{fig:selectiveds_compression}. Apart from bolstering the classification accuracy, selective downsampling furnishes data compression with regards to the overhead associated with training and testing datasets. Figure~\ref{fig:selectiveds_compression} portrays the variation of compression with increasing number of data samples. While we obtain savings of 84.87\% for the first 100 samples, we obtain 62.18\% and 54.61\% compression for the first 250 and 300 samples, respectively. This coupled with performance enhancement of kNN is beneficial in our endeavor to optimize in situ SE from an efficiency, hardware and cost point of view.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/9_ZnO_SelectiveDownsampling_Acc.png}
% \caption{Selective downsampling results of kNN classifier for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectiveds}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/10_ZnO_SelectiveDownsampling_AccDrop.png}
% \caption{Accuracy drop results of the kNN classifier for selective downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectivedsdrop}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/11_ZnO_CompressionSavings.png}
% \caption{Variation of compression with number of samples for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectivedscompression}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/12_ZnO_SelectiveDownsampling_Acc_Level1.png}
    \caption{}
    \label{fig:znoselectiveds_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/13_ZnO_SelectiveDownsampling_Acc_Level2.png}
    \caption{}
    \label{fig:znoselectiveds_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for selective downsampling of ZnO spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for selective downsampling of ZnO spectroscopic ellipsometry data.}
\label{fig:znoselectiveds_levels1-2}
\end{figure}

Next, we study the variation of level-1 accuracy and level-2 accuracy with thickness for the first 250 samples. Figure~\ref{fig:znoselectiveds_level1} shows the level-1 accuracy at different classes (each bin with 3 nm thickness) and Figure~\ref{fig:znoselectiveds_level2} the level-2 accuracy at different thickness values. From these graphs, it is evident that the classification performance of kNN degrades at higher thicknesses. The results obtained are similar to Figure~\ref{fig:znoimprovedlevel1} and Figure~\ref{fig:znoimprovedlevel2}. While we obtain level-1 prediction accuracy of 98.7\% for a thickness in bin [1 nm - 3 nm], the accuracy degrades to 50.98\% for a thickness in bin [43 nm - 44 nm]. The difference in accuracy scores at different thicknesses is clearly illustrated by Figure~\ref{fig:znoselectiveds_level2}; while accuracy is 99.05\% at t = 0, it drops to 10.53\% at t = 44 nm.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/12_ZnO_SelectiveDownsampling_Acc_Level1.png}
% \caption{Variation of accuracy of kNN classifier with classes for selective downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectivedslevel1}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/13_ZnO_SelectiveDownsampling_Acc_Level2.png}
% \caption{Variation of accuracy of kNN model with thickness for selective downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectivedslevel2}
% \vspace{-0.1in}
% \end{figure}

% \subsubsection{TiO2 Ellipsometry}
% \label{subsubsec:tio2results}

% \subsubsection{Al2O3 Ellipsometry}
% \label{subsubsec:al2o3results}

% \subsubsection{CeO2 Ellipsometry}
% \label{subsubsec:ceo2results}

\subsubsection{Expansion to other Chemistry}
\label{subsubsec:otherchemistryresults}

In this experiment, we explore other Chemistries, specifically TiO2 and Al2O3. Spectroscopic ellipsometry data for both these oxides are curated and collated using a procedure similar to ZnO and subsequently utilized to train and test ML algorithms. From our previous experiment on ZnO, it can be inferred that kNN is the ideal classifier among our suite of ML algorithms. Hence, we consider kNN as our classification model for both Chemistries.

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{Figures/TiO2/1_TiO2_kNN.png}
\caption{Accuracy results of kNN classifiers for TiO2 spectroscopic ellipsometry data.}
 \label{fig:tio2knnorig}
\vspace{-0.1in}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{Figures/Al2O3/1_Al2O3_kNN.png}
\caption{Accuracy results of kNN classifiers for AL2O3 spectroscopic ellipsometry data.}
 \label{fig:al2o3knnorig}
\vspace{-0.1in}
\end{figure}

Figure~\ref{fig:tio2knnorig} illustrates the baseline level-1 and level-2 accuracy scores of kNN on TiO2 SE data, which are 85.25\% and 71.44\%, respectively, using five neighbors. The improved classification performance of the kNN model is demonstrated in Figure~\ref{fig:tio2improved}, with level-1 accuracy now being 86.45\% and level-2 accuracy being 73.5\%, an increase of 1.2\% and 2.06\%, respectively. The baseline level-1 and level-2 accuracy scores of kNN on Al2O3 SE data are illustrated in Figure~\ref{fig:al2o3knnorig}. While the level-1 accuracy is 82.22\%, the level-2 accuracy is 65.35\%, and these scores are furnished using five neighbors in the kNN classifier. Figure~\ref{fig:tio2improved} demonstrates the improved classification performance of kNN, with level-1 and level-2 accuracy scores now being 83.65\% and 67.54\%, equivalent to an increase of 1.43\% and 2.19\%, respectively.

\begin{figure}[t!]
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/2_TiO2_kNNImproved.png}
    \caption{}
    \label{fig:tio2improved}
\end{subfigure}

\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/3_TiO2_kNN_Level1.png}
    \caption{}
    \label{fig:tio2improvedlevel1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/4_TiO2_kNN_Level2.png}
    \caption{}
    \label{fig:tio2improvedlevel2}
\end{subfigure}
\caption{(a) Accuracy results of the improved kNN algorithm for TiO2 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN classifier with classes for TiO2 spectroscopic ellipsometry data. (c) Variation of accuracy of kNN model with thickness for TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2improvedmodels_three}
\end{figure}

\begin{figure}[t!]
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/2_Al2O3_ImprovedModels.png}
    \caption{}
    \label{fig:al2o3improved}
\end{subfigure}

\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/3_Al2O3_kNN_Level1.png}
    \caption{}
    \label{fig:al2o3improvedlevel1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/4_Al2O3_kNN_Level2.png}
    \caption{}
    \label{fig:al2o3improvedlevel2}
\end{subfigure}
\caption{(a) Accuracy results of the improved kNN algorithm for Al2O3 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN classifier with classes for Al2O3 spectroscopic ellipsometry data. (c) Variation of accuracy of kNN model with thickness for Al2O3 spectroscopic ellipsometry data.}
\label{fig:al2o3improvedmodels_three}
\end{figure}

Figure~\ref{fig:tio2improvedlevel1} illustrates the accuracy of kNN at all classes for TiO2 data, and as evident from it, we generally witness reduced accuracy scores at classes comprising higher thicknesses. While class 0 ([1-3] nm) has the maximum accuracy of 99.09\%, class 14 ([43,44] nm) is associated with the minimum accuracy of 66.85\%. The accuracy for Al2O3 data deteriorates at higher classes, \emph{i.e.}, with an increase in thickness, as demonstrated by Figure~\ref{fig:al2o3improvedlevel1}. While class 0 ([1-3] nm) has the maximum accuracy of 97.83\%, class 10 ([31-33] nm) is associated with the minimum accuracy of 72.86\%. There is a considerable reduction in accuracy of around 32\% in TiO2 data and 25\% in Al2O3 data, which can mainly be attributed to the increased complexities associated with higher thicknesses. % There is a considerable reduction in accuracy of around 32\%, which can mainly be attributed to the fact that class 14 encompasses only one subclass ([43] nm), unlike the other classes, which consist of three subclasses. 
Next, we increase the granularity and examine kNN classification performance at each thickness, as depicted in Figure~\ref{fig:tio2improvedlevel2} for TiO2 and Figure~\ref{fig:al2o3improvedlevel2} for Al2O3 data. The accuracy values of the model for TiO2 data range between 97.41\% for 1 nm and 57.53\% for 38 nm, with the maximum thickness (43 nm) furnishing 78.92\% accuracy. On the other hand, for Al2O3 data, the kNN model furnish accuracy scores that range between 95.85\% for 1 nm and 47.98\% for 33 nm, with the maximum thickness (38 nm) furnishing 78.8\% accuracy. This is considered an outlier owing to the fact that the final class encompasses 1 subclass in TiO2 and 2 subclasses in AL2O3 data, as opposed to three subclasses in all other classes.

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/5_TiO2_Downsampling_Acc.png}
    \caption{}
    \label{fig:tio2dowsampling_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/6_TiO2_Downsampling_AccDrop.png}
    \caption{}
    \label{fig:tio2dowsampling_accdrop}
\end{subfigure}
\caption{(a) Random downsampling results of kNN classifier for TiO2 spectroscopic ellipsometry data. (b) Accuracy drop results of the kNN classifier for random downsampling of TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2downsamplingresults}
\end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/5_Al2O3_Downsampling_Acc.png}
    \caption{}
    \label{fig:al2o3dowsampling_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/6_Al2O3_Downsampling_AccDrop.png}
    \caption{}
    \label{fig:al2o3dowsampling_accdrop}
\end{subfigure}
\caption{(a) Random downsampling results of kNN classifier for Al2O3 spectroscopic ellipsometry data. (b) Accuracy drop results of the kNN classifier for random downsampling of Al2O3 spectroscopic ellipsometry data.}
\label{fig:al2o3downsamplingresults}
\end{figure}

As with the previous experiment, the downsampling rate is varied between 0 and 90\% and the classification performance of kNN algorithm is evaluated on the downsampled dataset. Figure~\ref{fig:tio2dowsampling_acc} and Figure~\ref{fig:al2o3dowsampling_acc} depict the variation of level-1 and level-2 accuracy at different downsampling rates for TiO2 and Al2O3 data, respectively. In the case of TiO2, the level-1 accuracy is generally resilient to donwnsampling, varying between 86.45\% at 0\% and 85.62\% at 85\%, witnessing a maximum accuracy drop of 0.8\%. The level-2 accuracy varies from 73.5\% at 0\% downsampling to 67.02\% at 90\% downsampling. In the case of Al2O3, level-1 accuracy varies between 83.65\% at 0\% and 81.84\% at 90\%, witnessing a modest accuracy drop of 1.81\%. Meanwhile, level-2 accuracy varies from 67.54\% to 63.71\% for the same range.

Figure~\ref{fig:tio2dowsampling_accdrop} and Figure~\ref{fig:al2o3dowsampling_accdrop} illustrate the accuracy drop associated with random downsampling for TiO2 and Al2O3, respectively. In the case of TiO2, random downsampling induces a larger degradation in level-2 accuracy, \emph{i.e.}, 7.35\% drop in classification accuracy of the kNN model. However, the accuracy drops are modest at both levels until 50\% downsampling, with the performance degradation at level-1 and level-2 for 50\% downsampling rate being 2.11\% and 2.4\%, respectively. The trend is similar for Al2O3 data, with the maximum accuracy drop at level 1 and level 2 being 3.83\% and 1.81\%, respectively. Furthermore, we obtain negligible accuracy drop until 60\% downsampling rate. Hence, we can once again infer the redundancy present in the SE dataset.

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/7_TiO2_Downsampling_Acc_Level1.png}
    \caption{}
    \label{fig:tio2downsamling_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/8_TiO2_Downsampling_Acc_Level2.png}
    \caption{}
    \label{fig:tio2downsamling_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for random downsampling of TiO2 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for random downsampling of TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2randomdownsamplingresults}
\end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/7_Al2O3_Downsampling_Acc_Level1.png}
    \caption{}
    \label{fig:al2o3downsamling_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/8_Al2O3_Downsampling_Acc_Level2.png}
    \caption{}
    \label{fig:al2o3downsamling_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for random downsampling of Al2O3 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for random downsampling of Al2O3 spectroscopic ellipsometry data.}
\label{fig:al2o3randomdownsamplingresults}
\end{figure}

For TiO2 data, the level-1 and level-2 accuracy scores of random downsampling are illustrated by Figure~\ref{fig:tio2downsamling_level1} and Figure~\ref{fig:tio2downsamling_level2}, respectively, and, from these graphs, it is evident that the classification accuracy of our model deteriorates at higher thicknesses, irrespective of the downsampling rate. For example, with 90\% downsampling of SE data, level-1 prediction accuracy drops from 93.4\% for a thickness in bin [1 nm - 3 nm] to 84\% and 43.64\% for thicknesses in bin [40 nm - 42 nm] and [43 nm], respectively.

Figure~\ref{fig:al2o3downsamling_level1} and Figure~\ref{fig:al2o3downsamling_level2} demonstrate the level-1 and level-2 accuracy scores for Al2O3 data, which are similar to TiO2.  At 90\% downsampling rate, level-1 accuracy drops from 96.3\% for a thickness in bin [1 nm - 3 nm] to 68.8\% for thickness in bin [28 nm - 30 nm]. Hence, this inherent redundancy in both dataset reinforces our motivation to perform selective downsampling.

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/9_TiO2_SelectiveDownsampling_Acc.png}
    \caption{}
    \label{fig:tio2selectiveds_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/11_TiO2_CompressionSavings.png}
    \caption{}
    \label{fig:tio2selectiveds_compression}
\end{subfigure}
\caption{(a) Selective downsampling results of kNN classifier for TiO2 spectroscopic ellipsometry data. (b) Variation of compression with number of samples for TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2selectivedsresults}
\end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/9_Al2O3_SelectiveDownsampling_Acc.png}
    \caption{}
    \label{fig:al2o3selectiveds_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/11_Al2O3_CompressionSavings.png}
    \caption{}
    \label{fig:al2o3selectiveds_compression}
\end{subfigure}
\caption{(a) Selective downsampling results of kNN classifier for Al2O3 spectroscopic ellipsometry data. (b) Variation of compression with number of samples for Al2O3 spectroscopic ellipsometry data.}
\label{fig:al2o3selectivedsresults}
\end{figure}

In the selective downsampling analysis, we consider N ranging from 100 to 300, in step sizes of 50, which corresponds to a spectral window from 271 nm to 427 nm for the first 100, and from 271 nm to 743 nm for first 300, in step sizes of 76 nm. Figure~\ref{fig:tio2selectiveds_acc} demonstrates the variation of level-1 and level-2 classification accuracy scores for TiO2 data. While we obtain the lowest scores of 82.21\% at level-1 and 73.38\% at level-2 for the first 100 samples, improved classification performance is produced at higher values of N. The best level-1 accuracy and level-2 accuracy are 88.76\% and 85.14\%, which are furnished when the first 300 samples constitute the dataset (opposed to 86.45\% level-1 and 73.5\% level-2 accuracies when no downsampling is performed, as shown in Figure~\ref{fig:tio2improvedmodels_three}). This approach of selective downsampling provides results that exceed the baseline accuracy scores of the kNN model, by 2.31\% at level-1 and 11.64\% at level-2. % This enhanced performance is accompanied with reduced data dimensionality (54.61\% compression for the first 300 samples), as illustrated in Figure~\ref{fig:tio2selectiveds_compression}. 

In the case of Al2O3 spectroscopic ellipsometry, the best level-1 and level-2 accuracy scores of 87.02\% and 79.17\% are furnished for the first 300 samples, as illustrated in Figure~\ref{fig:al2o3selectiveds_acc}, which is an improvement of 3.4\% at level 1 and 11.63\% at level-2. In both cases, the enhanced classification performance is accompanied with reduced data dimensionality (54.61\% compression for the first 300 samples), as illustrated in Figure~\ref{fig:tio2selectiveds_compression} and Figure~\ref{fig:al2o3selectiveds_compression}. Such an approach facilitates an efficient, simple, and cost-effective thickness estimation from SE data.

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/12_TiO2_SelectiveDownsampling_Acc_Level1.png}
    \caption{}
    \label{fig:tio2selectiveds_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/13_TiO2_SelectiveDownsampling_Acc_Level2.png}
    \caption{}
    \label{fig:tio2selectiveds_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for selective downsampling of TiO2 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for selective downsampling of TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2selectiveds_levels1-2}
\end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/12_Al2O3_SelectiveDownsampling_Acc_Level1.png}
    \caption{}
    \label{fig:al2o3selectiveds_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Al2O3/13_Al2O3_SelectiveDownsampling_Acc_Level2.png}
    \caption{}
    \label{fig:al2o3selectiveds_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for selective downsampling of Al2O3 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for selective downsampling of Al2O3 spectroscopic ellipsometry data.}
\label{fig:al2o3selectiveds_levels1-2}
\end{figure}

The variation of level-1 accuracy and level-2 accuracy with thickness for the first 300 samples are illustrated in Figure~\ref{fig:tio2selectiveds_level1} and Figure~\ref{fig:tio2selectiveds_level2}, respectively, for TiO2 data. While we obtain level-1 prediction accuracy of 98.1\% for a thickness in bin [1 nm - 3 nm], the accuracy degrades to 76.11\% for a thickness in bin [43 nm]. The difference in accuracy scores at different thicknesses is clearly illustrated by Figure~\ref{fig:tio2selectiveds_level2}; accuracy varies from 98.5\% at t = 0 to 84.21\% at t = 43 nm.

Figure~\ref{fig:al2o3selectiveds_level1} and Figure~\ref{fig:al2o3selectiveds_level2} demonstrate the variation of level-1 and level-2 accuracy for Al2O3 data. While level-1 accuracy varies from 97.28\% for a thickness in bin [1 nm - 3 nm] to 80.4\% for a thickness in bin [25 nm - 27 nm], level-2 accuracy varies from 93.16\% at t = 0 to 65.1\% at t = 33 nm.

\subsubsection{Transfer Learning}
\label{subsubsec:transferlearningresults}

==> Sections/results_backup.tex <==
\section{Experiments}
\label{sec:results}

\subsection{Experimental Setup}
\label{sec:setup}

Text by UCF.

\subsection{Results}
\label{subsec:results}

\subsubsection{ZnO Ellipsometry}
\label{subsubsec:znoresults}

The first case study compares the performance of the various ML algorithms, as demonstrated in Figure\ref{fig:znoallclassifiers}. The percent accuracy (Y-axis) illustrates the probability of each model to classify a datapoint into one of the fifteen classes of the curated dataset to within ± 1.5 nm accuracy, i.e., level-1 classification. kNN furnishes the best accuracy score, where each datapoint is classified with a confidence of 87.54\% using five neighbors~\textcolor{orange}{cite here}. SVM, DT, and RF report acceptable results, comparable to kNN, of 83.77\%, 84.54\%, and 86.79\%, respectively. SVM uses a radial basis function of degree three as its kernel, along with a regularization coefficient of value 1. RF is an ensemble of decision trees, and like DT, requires a minimum of two samples to split an internal node. The maximum depth of the tree is not specified in either algorithm, implying that the tree can expand until all datapoints are accounted for. In this experiment, we consider 40 trees in RF. LR, on the other hand, uses a regularization coefficient of value 1 and Limited-memory Broyden–Fletcher–Goldfarb–Shanno (lbfgs) optimization technique36 to calculate the parameter weights that minimize the cost function.

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{Figures/ZnO/1_ZnO_AllClassifiers.png}
\caption{Accuracy results of various Machine Learning classifiers for ZnO spectroscopic ellipsometry data.}
 \label{fig:znoallclassifiers}
\vspace{-0.1in}
\end{figure}

LR performs the worst among all the models, producing a score of 40.74\%. This can be attributed to LR being inept at solving non-linear problems owing to its linear decision surface, the requirement of having an exhaustive dataset, and its sensitivity of outliers in the dataset. Owing to its low accuracy score, LR is not considered for future experiments. Additionally, SVM too is excluded from subsequent case studies for two reasons, the first being its high training time and the second its sub-par classification performance.

The second case study evaluates the performances of the three best algorithms, DT, RF and kNN, with increasing granularity in the prediction of film thickness. These results assume importance from a process perspective since it is important to understand the uncertainty in accuracy (i.e., delta thickness) that is inherently present in a ML algorithm and the uncertainty that is propagated as a function of the true physical thickness of the film.

Accordingly, accuracy scores of each model are as illustrated in Figure~\ref{fig:znoimproved} at both level-1 and level-2. We have updated the hyperparameters of the models to bolster classification performance of each model. Increasing the number of neighbors from 5 to 21 improves the performance of kNN from 87.54\% (as shown in Figure~\ref{fig:znoallclassifiers}) to 88.65\% resulting in an enhancement of 1.11\%. The number of trees in RF is increased from 40 to 100, which furnishes an accuracy of 87.25\% vs. 86.79\%. DT retains the same set of hyperparameters as before, which were optimized to produce best performance, and thus produces the same accuracy score of 84.54\%.  

\begin{figure}[t!]
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/2_ZnO_ImprovedModels.png}
    \caption{}
    \label{fig:znoimproved}
\end{subfigure}

\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/3_ZnO_kNN_Level1.png}
    \caption{}
    \label{fig:znoimprovedlevel1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/4_ZnO_kNN_Level2.png}
    \caption{}
    \label{fig:znoimprovedlevel2}
\end{subfigure}
\caption{(a) Accuracy results of the improved Machine Learning classifiers for ZnO spectroscopic ellipsometry data. (b) Variation of accuracy of kNN classifier with classes for ZnO spectroscopic ellipsometry data. (c) Variation of accuracy of kNN model with thickness for ZnO spectroscopic ellipsometry data.}
\label{fig:znoimprovedmodels_three}
\end{figure}

Apart from refining the models, we also analyze their level-2 accuracy scores. It is intuitive to understand how level-1 classification (wider, 3 nm range) may result in higher accuracy compared to level-2 classification (narrower, 1 nm range). As depicted in Figure~\ref{fig:znoimproved}, kNN again furnishes the best results of 73.83\%, while RF and DT produce scores of 71.56\% and 67.45\%, respectively.  

Since these results reflect the overall classification performance, averaged over all classes and subclasses, there is no information regarding the accuracy scores at specific classes or thicknesses. Hence, we next examine level-1 accuracy and level-2 accuracy by analyzing model performance at each class and thickness, respectively.  

Figure~\ref{fig:znoimprovedlevel1} illustrates the accuracy of kNN at all classes, and as evident from it, we generally witness reduced accuracy scores at classes comprising higher thicknesses. While class 0 ([1-3] nm) has the maximum accuracy of 98.58\%, class 14 ([43,44] nm) is associated with the minimum accuracy of 53.36\%. There is a considerable reduction in accuracy of around 30\%, which can mainly be attributed to the fact that class 14 encompasses only two subclasses ([43-44] nm), unlike the other classes, which consist of three subclasses. Moreover, since the ALD process is terminated at 51.17 min, as soon as a film of 44 nm thickness is obtained, we have access to limited datapoints for this thickness. Next, we increase the granularity and examine kNN classification performance at each thickness, as depicted in Figure~\ref{fig:znoimprovedlevel2}. The accuracy values of the model range between 97.78\% for 1 nm and 3.85\% for 44 nm. Although the general trend is negative, there are a few outliers (such as 39 nm and 42 nm) that produce high accuracy scores. The performance degradation at higher thicknesses may be attributed to the amplification of spectral features in $\Psi$ and $\Delta$, (i.e., peaks and valleys in \textcolor{orange}{Figure 3A, B)} which hinder the learning stage of the models and degrade their classification performance.

% \begin{figure}[t!]
% \centering
%%\subfloat[]{\label{main:c}\includegraphics[scale=.5]{Figures/2_ZnO_ImprovedModels.png}}
% \subfloat[]{\label{main:c}\includegraphics[width=\linewidth]{Figures/2_ZnO_ImprovedModels.png}}
% \begin{minipage}{.5\linewidth}
% \centering
% \subfloat[]{\label{main:a}\includegraphics[width=0.5\linewidth]{Figures/3_ZnO_kNN_Level1.png}}
% \end{minipage}%
% \begin{minipage}{.5\linewidth}
% \centering
% \subfloat[]{\label{main:b}\includegraphics[width=0.5\linewidth]{Figures/4_ZnO_kNN_Level2.png}}
% \end{minipage}\par\medskip
% \caption{my fig}
% \label{fig:main}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/2_ZnO_ImprovedModels.png}
% \caption{Accuracy results of the improved Machine Learning classifiers for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoimprovedmodels}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/3_ZnO_kNN_Level1.png}
% \caption{Variation of accuracy of kNN classifier with classes for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znolevel1}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/4_ZnO_kNN_Level2.png}
% \caption{Variation of accuracy of kNN model with thickness for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znolevel2}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/5_ZnO_Downsampling_Acc.png}
    \caption{}
    \label{fig:znodowsampling_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/6_ZnO_Downsampling_AccDrop.png}
    \caption{}
    \label{fig:znodowsampling_accdrop}
\end{subfigure}
\caption{(a) Random downsampling results of kNN classifier for ZnO spectroscopic ellipsometry data. (b) Accuracy drop results of the kNN classifier for random downsampling of ZnO spectroscopic ellipsometry data.}
\label{fig:downsamplingresults}
\end{figure}

The third case study describes the results of downsampling data, i.e., random $\Psi$ and $\Delta$ values are removed from the curated dataset. Here, we seek to understand how limited spectroscopic data might impact ML prediction accuracy. In the ultimate limit, where only one wavelength (as is the case for single wavelength ellipsometry) is present, might ML accurately predict film thickness? The results assume importance because limited data might indicate avenues for faster data acquisition, reduced hardware complexity (i.e., costs) and therefore, easier integration of SE for \textit{in situ} monitoring of thin film deposition processes, in general. 

The downsampling rate is varied between 0 and 90\% and the performance of the best performing algorithm – the kNN algorithm, is evaluated on the downsampled dataset. Figure~\ref{fig:znodowsampling_acc} depicts the variation of level-1 and level-2 accuracy at different downsampling rates. The level-1 accuracy is generally resilient to donwnsampling, varying between 88.65\% at 0\% and 85.67\% at 85\%, witnessing a maximum accuracy drop of 2.98\%. The level-2 accuracy varies from 73.83\% at 0\% downsampling to 65.46\% at 90\% downsampling. This is an important result as it indicates that thickness prediction via ML can be effectively accurate to within ± 1.5 nm uncertainty (i.e., level-1) of a ZnO film $\leq44 nm$, even if 90\% of the spectral data is eliminated.  

On the other hand, Figure~\ref{fig:znodowsampling_accdrop} shows that downsampling induces a larger degradation in level-2 accuracy. This is equivalent to 8.37\% drop in classification accuracy of the kNN model. However, the accuracy drops are relatively low at both levels until 50\% downsampling. The performance degradation at level-1 and level-2 for 50\% downsampling rate is 0.54\% and 2\%, respectively. These results are indicative of possible redundancy in the dataset with regards to $\Psi$ and $\Delta$ samples. 

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/5_ZnO_Downsampling_Acc.png}
% \caption{Random downsampling results of kNN classifier for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znodownsampling}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/6_ZnO_Downsampling_AccDrop.png}
% \caption{Accuracy drop results of the kNN classifier for random downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znodownsamplingdrop}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/7_ZnO_Downsampling_Acc_Level1.png}
    \caption{}
    \label{fig:znodownsamling_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/8_ZnO_Downsampling_Acc_Level2.png}
    \caption{}
    \label{fig:znodownsamling_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for random downsampling of ZnO spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for random downsampling of ZnO spectroscopic ellipsometry data.}
\label{fig:randomdownsamplingresults}
\end{figure}

We further study the variation of level-1 accuracy and level-2 accuracy with thickness at select downsampling rates of 10\%, 30\%, 50\%, 70\%, and 90\%. Figure~\ref{fig:znodownsamling_level1} shows the level-1 accuracy at different classes (each bin with 3 nm thickness) and Figure~\ref{fig:znodownsamling_level2} the level-2 accuracy at different thickness values. From these graphs, it is evident that the classification performance of kNN degrades at higher thicknesses, irrespective of the random downsampling rate. For example, with 90\% downsampling of SE data, level-1 prediction accuracy drops from 97.01\% for a thickness in bin [4 nm - 6 nm] to 77.55\% for a thickness in bin [40 nm - 42 nm]. Thus, it is the actual physical thickness of the film predicted using ML that can make a difference to the predictive accuracy. This result bodes well for ML algorithms to predict thickness of ultrathin films ($\leq10 nm$) which is always a challenge for SE data analysis. Finally, it can be inferred that the dataset has redundancy that can be eliminated without inducing significant performance degradation. Hence, this motivates us to pursue selective downsampling and explore the connection, if any, between specific $\Psi$ and $\Delta$ samples and classification accuracy.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/7_ZnO_Downsampling_Acc_Level1.png}
% \caption{Variation of accuracy of kNN classifier with classes for random downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znodownsamplinglevel1}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/8_ZnO_Downsampling_Acc_Level2.png}
% \caption{Variation of accuracy of kNN model with thickness for random downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znodownsamplinglevel2}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/9_ZnO_SelectiveDownsampling_Acc.png}
    \caption{}
    \label{fig:selectiveds_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/11_ZnO_CompressionSavings.png}
    \caption{}
    \label{fig:selectiveds_compression}
\end{subfigure}
\caption{(a) Selective downsampling results of kNN classifier for ZnO spectroscopic ellipsometry data. (b) Variation of compression with number of samples for ZnO spectroscopic ellipsometry data.}
\label{fig:selectivedsresults}
\end{figure}

The ultimate objective of an ML algorithm would be to determine thickness from minimal, perhaps few and discrete, wavelength based ellipsometry data. Therefore, the fourth case study involves selective (i.e., non-random) downsampling of $\Psi$ and $\Delta$ values in the curated dataset. We select the first ‘N’ samples from each class and subclass, starting from 271 nm and up, while eliminating the rest. This is shown in Figure~\textcolor{orange}{include figure} which serves to remind the reader of the $\Psi$ and $\Delta$ values of a single spectrum (i.e., related to a fixed thickness). Features such as peaks and valleys appear in the spectra for wavelengths $\leq500 nm$. It is important to note that the $\Psi$ and $\Delta$ are experimentally measured raw data and no modeling effort has been expended to modify the data.  

In this analysis, we consider N ranging from 100 to 300, in step sizes of 50. This corresponds to a spectral window from 271 nm to 427 nm for the first 100, and from 271 nm to 743 nm for first 300, in step sizes of 76 nm. From Figure~\ref{fig:znoselectivedscompression}, an estimate can be made that the first – 300 data points still constitutes a fraction (45.39\%) of the total data collected. 

This downsampled dataset is utilized to train and evaluate kNN, which, in the previous three case studies, has furnished the best results. Figure~\ref{fig:selectiveds_acc} shows the variation of level-1 and level-2 classification accuracy scores. While we obtain the lowest scores of 78.25\% at level-1 and 67.13\% at level-2 for the first 100 samples, improved classification performance is produced at higher values of N. The best level-1 accuracy and level-2 accuracy are 88.63\% and 80.04\%, which are furnished when the first 250 and 300 samples, respectively, constitute the dataset (opposed to 88.65\% level-1 and 73.87\% level-2 accuracies when no downsampling is performed, as shown in Figure~\ref{fig:znoimprovedmodels_three}). This approach of selective downsampling provides results that exceed the baseline accuracy scores of the kNN model, by 6.21\% at level-2.

Another benefit of selective downsampling is illustrated in Figure~\ref{fig:selectiveds_compression}. Apart from bolstering the classification accuracy, selective downsampling furnishes data compression with regards to the overhead associated with training and testing datasets. Figure~\ref{fig:selectiveds_compression} portrays the variation of compression with increasing number of data samples. While we obtain savings of 84.87\% for the first 100 samples, we obtain 62.18\% and 54.61\% compression for the first 250 and 300 samples, respectively. This coupled with performance enhancement of kNN is beneficial in our endeavor to optimize in situ SE from an efficiency, hardware and cost point of view.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/9_ZnO_SelectiveDownsampling_Acc.png}
% \caption{Selective downsampling results of kNN classifier for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectiveds}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/10_ZnO_SelectiveDownsampling_AccDrop.png}
% \caption{Accuracy drop results of the kNN classifier for selective downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectivedsdrop}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/11_ZnO_CompressionSavings.png}
% \caption{Variation of compression with number of samples for ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectivedscompression}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/12_ZnO_SelectiveDownsampling_Acc_Level1.png}
    \caption{}
    \label{fig:znoselectiveds_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ZnO/13_ZnO_SelectiveDownsampling_Acc_Level2.png}
    \caption{}
    \label{fig:znoselectiveds_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for selective downsampling of ZnO spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for selective downsampling of ZnO spectroscopic ellipsometry data.}
\label{fig:znoselectiveds_levels1-2}
\end{figure}

Next, we study the variation of level-1 accuracy and level-2 accuracy with thickness for the first 250 samples. Figure~\ref{fig:znoselectiveds_level1} shows the level-1 accuracy at different classes (each bin with 3 nm thickness) and Figure~\ref{fig:znoselectiveds_level2} the level-2 accuracy at different thickness values. From these graphs, it is evident that the classification performance of kNN degrades at higher thicknesses. The results obtained are similar to Figure~\ref{fig:znoimprovedlevel1} and Figure~\ref{fig:znoimprovedlevel2}. While we obtain level-1 prediction accuracy of 98.7\% for a thickness in bin [1 nm - 3 nm], the accuracy degrades to 50.98\% for a thickness in bin [43 nm - 44 nm]. The difference in accuracy scores at different thicknesses is clearly illustrated by Figure~\ref{fig:znoselectiveds_level2}; while accuracy is 99.05\% at t = 0, it drops to 10.53\% at t = 44 nm.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/12_ZnO_SelectiveDownsampling_Acc_Level1.png}
% \caption{Variation of accuracy of kNN classifier with classes for selective downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectivedslevel1}
% \vspace{-0.1in}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{Figures/13_ZnO_SelectiveDownsampling_Acc_Level2.png}
% \caption{Variation of accuracy of kNN model with thickness for selective downsampling of ZnO spectroscopic ellipsometry data.}
%  \label{fig:znoselectivedslevel2}
% \vspace{-0.1in}
% \end{figure}

% \subsubsection{TiO2 Ellipsometry}
% \label{subsubsec:tio2results}

% \subsubsection{Al2O3 Ellipsometry}
% \label{subsubsec:al2o3results}

% \subsubsection{CeO2 Ellipsometry}
% \label{subsubsec:ceo2results}

\subsubsection{Expansion to other Chemistry}
\label{subsubsec:otherchemistryresults}

In this experiment, we explore other Chemistries, specifically TiO2 and Al2O3. Spectroscopic ellipsometry data for both these oxides are curated and collated using a procedure similar to ZnO and subsequently utilized to train and test ML algorithms. From our previous experiment on ZnO, it can be inferred that kNN is the ideal classifier among our suite of ML algorithms. Hence, we consider kNN as our classification model for both Chemistries.

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{Figures/TiO2/1_TiO2_kNN.png}
\caption{Accuracy results of kNN classifiers for TiO2 spectroscopic ellipsometry data.}
 \label{fig:tio2knnorig}
\vspace{-0.1in}
\end{figure}

Figure~\ref{fig:tio2knnorig} illustrates the baseline level-1 and level-2 accuracy scores of kNN on TiO2 SE data, which are 85.25\% and 71.44\%, respectively, using five neighbors. The improved classification performance of the kNN model is demosntrated in Figure~\ref{fig:tio2improved}, with level-1 accuracy now being 86.45\% and level-2 accuracy being 73.5\%, an increase of 1.2\% and 2.06\%, respectively. 

\begin{figure}[t!]
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/2_TiO2_kNNImproved.png}
    \caption{}
    \label{fig:tio2improved}
\end{subfigure}

\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/3_TiO2_kNN_Level1.png}
    \caption{}
    \label{fig:tio2improvedlevel1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/4_TiO2_kNN_Level2.png}
    \caption{}
    \label{fig:tio2improvedlevel2}
\end{subfigure}
\caption{(a) Accuracy results of the improved kNN algorithm for TiO2 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN classifier with classes for TiO2 spectroscopic ellipsometry data. (c) Variation of accuracy of kNN model with thickness for TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2improvedmodels_three}
\end{figure}

Figure~\ref{fig:tio2improvedlevel1} illustrates the accuracy of kNN at all classes, and as evident from it, we generally witness reduced accuracy scores at classes comprising higher thicknesses. While class 0 ([1-3] nm) has the maximum accuracy of 99.09\%, class 14 ([43,44] nm) is associated with the minimum accuracy of 66.85\%. There is a considerable reduction in accuracy of around 32\%, which can mainly be attributed to the fact that class 14 encompasses only one subclass ([43] nm), unlike the other classes, which consist of three subclasses. Next, we increase the granularity and examine kNN classification performance at each thickness, as depicted in Figure~\ref{fig:tio2improvedlevel2}. The accuracy values of the model range between 97.41\% for 1 nm and 57.53\% for 38 nm, with the maximum thickness (43 nm) furnishing 78.92\% accuracy. This is considered an outlier owing to the fact that class 14 encompasses only 1 subclass.

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/5_TiO2_Downsampling_Acc.png}
    \caption{}
    \label{fig:tio2dowsampling_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/6_TiO2_Downsampling_AccDrop.png}
    \caption{}
    \label{fig:tio2dowsampling_accdrop}
\end{subfigure}
\caption{(a) Random downsampling results of kNN classifier for TiO2 spectroscopic ellipsometry data. (b) Accuracy drop results of the kNN classifier for random downsampling of TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2downsamplingresults}
\end{figure}

As with the previous experiment, the downsampling rate is varied between 0 and 90\% and the classification performance of kNN algorithm is evaluated on the downsampled dataset. Figure~\ref{fig:tio2dowsampling_acc} depicts the variation of level-1 and level-2 accuracy at different downsampling rates. The level-1 accuracy is generally resilient to donwnsampling, varying between 86.45\% at 0\% and 85.62\% at 85\%, witnessing a maximum accuracy drop of 0.8\%. The level-2 accuracy varies from 73.5\% at 0\% downsampling to 67.02\% at 90\% downsampling. On the other hand, Figure~\ref{fig:tio2dowsampling_accdrop} shows that downsampling induces a larger degradation in level-2 accuracy. This is equivalent to 7.35\% drop in classification accuracy of the kNN model. However, the accuracy drops are modest at both levels until 50\% downsampling. The performance degradation at level-1 and level-2 for 50\% downsampling rate is 2.11\% and 2.4\%, respectively. These results are indicative of possible redundancy in the dataset with regards to $\Psi$ and $\Delta$ samples. 

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/7_TiO2_Downsampling_Acc_Level1.png}
    \caption{}
    \label{fig:tio2downsamling_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/8_TiO2_Downsampling_Acc_Level2.png}
    \caption{}
    \label{fig:tio2downsamling_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for random downsampling of TiO2 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for random downsampling of TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2randomdownsamplingresults}
\end{figure}

We further study the variation of level-1 accuracy and level-2 accuracy with thickness at select downsampling rates of 10\%, 30\%, 50\%, 70\%, and 90\%. Figure~\ref{fig:znodownsamling_level1} shows the level-1 accuracy at different classes (each bin with 3 nm thickness) and Figure~\ref{fig:znodownsamling_level2} the level-2 accuracy at different thickness values. From these graphs, it is evident that the classification performance of kNN degrades at higher thicknesses, irrespective of the random downsampling rate. For example, with 90\% downsampling of SE data, level-1 prediction accuracy drops from 97.01\% for a thickness in bin [4 nm - 6 nm] to 77.55\% for a thickness in bin [40 nm - 42 nm]. Thus, it is the actual physical thickness of the film predicted using ML that can make a difference to the predictive accuracy. This result bodes well for ML algorithms to predict thickness of ultrathin films ($\leq10 nm$) which is always a challenge for SE data analysis. Finally, it can be inferred that the dataset has redundancy that can be eliminated without inducing significant performance degradation. Hence, this motivates us to pursue selective downsampling and explore the connection, if any, between specific $\Psi$ and $\Delta$ samples and classification accuracy.

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/9_TiO2_SelectiveDownsampling_Acc.png}
    \caption{}
    \label{fig:tio2selectiveds_acc}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/11_TiO2_CompressionSavings.png}
    \caption{}
    \label{fig:tio2selectiveds_compression}
\end{subfigure}
\caption{(a) Selective downsampling results of kNN classifier for TiO2 spectroscopic ellipsometry data. (b) Variation of compression with number of samples for TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2selectivedsresults}
\end{figure}

The ultimate objective of an ML algorithm would be to determine thickness from minimal, perhaps few and discrete, wavelength based ellipsometry data. Therefore, the fourth case study involves selective (i.e., non-random) downsampling of $\Psi$ and $\Delta$ values in the curated dataset. We select the first ‘N’ samples from each class and subclass, starting from 271 nm and up, while eliminating the rest. This is shown in Figure~\textcolor{orange}{include figure} which serves to remind the reader of the $\Psi$ and $\Delta$ values of a single spectrum (i.e., related to a fixed thickness). Features such as peaks and valleys appear in the spectra for wavelengths $\leq500 nm$. It is important to note that the $\Psi$ and $\Delta$ are experimentally measured raw data and no modeling effort has been expended to modify the data.  

In this analysis, we consider N ranging from 100 to 300, in step sizes of 50. This corresponds to a spectral window from 271 nm to 427 nm for the first 100, and from 271 nm to 743 nm for first 300, in step sizes of 76 nm. From Figure~\ref{fig:znoselectivedscompression}, an estimate can be made that the first – 300 data points still constitutes a fraction (45.39\%) of the total data collected. 

This downsampled dataset is utilized to train and evaluate kNN, which, in the previous three case studies, has furnished the best results. Figure~\ref{fig:selectiveds_acc} shows the variation of level-1 and level-2 classification accuracy scores. While we obtain the lowest scores of 78.25\% at level-1 and 67.13\% at level-2 for the first 100 samples, improved classification performance is produced at higher values of N. The best level-1 accuracy and level-2 accuracy are 88.63\% and 80.04\%, which are furnished when the first 250 and 300 samples, respectively, constitute the dataset (opposed to 88.65\% level-1 and 73.87\% level-2 accuracies when no downsampling is performed, as shown in Figure~\ref{fig:znoimprovedmodels_three}). This approach of selective downsampling provides results that exceed the baseline accuracy scores of the kNN model, by 6.21\% at level-2.

Another benefit of selective downsampling is illustrated in Figure~\ref{fig:selectiveds_compression}. Apart from bolstering the classification accuracy, selective downsampling furnishes data compression with regards to the overhead associated with training and testing datasets. Figure~\ref{fig:selectiveds_compression} portrays the variation of compression with increasing number of data samples. While we obtain savings of 84.87\% for the first 100 samples, we obtain 62.18\% and 54.61\% compression for the first 250 and 300 samples, respectively. This coupled with performance enhancement of kNN is beneficial in our endeavor to optimize in situ SE from an efficiency, hardware and cost point of view.

\begin{figure}[t!]
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/12_TiO2_SelectiveDownsampling_Acc_Level1.png}
    \caption{}
    \label{fig:tio2selectiveds_level1}
\end{subfigure}%
~
\begin{subfigure}{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/TiO2/13_TiO2_SelectiveDownsampling_Acc_Level2.png}
    \caption{}
    \label{fig:tio2selectiveds_level2}
\end{subfigure}
\caption{(a) Variation of accuracy of kNN classifier with classes for selective downsampling of TiO2 spectroscopic ellipsometry data. (b) Variation of accuracy of kNN model with thickness for selective downsampling of TiO2 spectroscopic ellipsometry data.}
\label{fig:tio2selectiveds_levels1-2}
\end{figure}

Next, we study the variation of level-1 accuracy and level-2 accuracy with thickness for the first 250 samples. Figure~\ref{fig:znoselectiveds_level1} shows the level-1 accuracy at different classes (each bin with 3 nm thickness) and Figure~\ref{fig:znoselectiveds_level2} the level-2 accuracy at different thickness values. From these graphs, it is evident that the classification performance of kNN degrades at higher thicknesses. The results obtained are similar to Figure~\ref{fig:znoimprovedlevel1} and Figure~\ref{fig:znoimprovedlevel2}. While we obtain level-1 prediction accuracy of 98.7\% for a thickness in bin [1 nm - 3 nm], the accuracy degrades to 50.98\% for a thickness in bin [43 nm - 44 nm]. The difference in accuracy scores at different thicknesses is clearly illustrated by Figure~\ref{fig:znoselectiveds_level2}; while accuracy is 99.05\% at t = 0, it drops to 10.53\% at t = 44 nm.

\subsubsection{Transfer Learning}
\label{subsubsec:transferlearningresults}
